Parity to Safety in Polynomial Time for Pushdown and Collapsible Pushdown Systems

We give a direct polynomial-time reduction from parity games played over the configuration graphs of collapsible pushdown systems to safety games played over the same class of graphs. That a polynomial-time reduction would exist was known since both problems are complete for the same complexity class. Coming up with a direct reduction, however, has been an open problem. Our solution to the puzzle brings together a number of techniques for pushdown games and adds three new ones. This work contributes to a recent trend of liveness to safety reductions which allow the advanced state-of-the-art in safety checking to be used for more expressive specifications.

==> counterreduction_unused.tex <==

When incrementing counter $\counter_\rank$ we will rest all counters
That is, for all $\rank$ (including even ranks)
\begin{multline*}
    
    \\
    =
    \begin{cases}
        \overflow
        &
        }
        \\
        \tup{\counter'_1, \counter'_3, \ldots, \counter'_\maxrank}
        &
        \text{otherwise}
    \end{cases}
\end{multline*}


, $\chb' = \tup{\chb, \countervec}$, and 
        $\rank = \ap{\rankf}{\control'}$.
        Note that $\countervec$ is the same as in $\cha'.

        
        $\tup{\control, \cha, \rew{\chb}, \control'} \in \cpdsrules$,
        $\rank = \ap{\rankf}{\control'}$,
        $\cha' = \tup{\cha, \countervec}$, and
        $\chb' = \tup{\chb, \countervec}$.

==> orderreduction_unused.tex <==
%, where $\popguess^{\star}$ does not clash with any obligation in the de used is a fresh obligation (and hence universally. 
%This means the component is (implicitly) universally quantified and the rule exist for all choices of $\popguess^{\star}$. 
%That is $\cpdsrules'$ (only) contains all rules of the following forms.

 %       with
 %           $\cha' = \cha$ or $\cha' = \tup{\cha, \popguess'}$.
 %       Note that $\popguess'$ is not specified, which meansthe transition exists
 %       for all choices of $\popguess'$.


==> outline_unused.tex <==
In the following sections, from parity game over a rank-aware CPDS $\game$ we will use two reductions,





Whereas the proof of t
For



%  note that $$ With the previous previous lemma, equivalence means we ah

That the resulting game is equivalent  result is equivalent in 
In combination with Equivalence 



Note that, with the previous lemma, a
Together 

The function $\polyred{}$ used in the main theorem computes $\ap{\polyred{}}{\game}=\ap{\polyred{\bound}}{\game}$ with $\bound$ the $n$-fold exponential value from Lemma~\ref{lem:parityvssafety}.
Hence, to 

 in polynomial time.


We note that the 
The parameter $\bound$ is a bound on the counter values, and the goal of the \theeplayer in the safety game is 

give a function 

and encodes a counter for each odd rank of the parity game into the stack characters of the CPDS up to the bound $\bound$.
Essentially, we observe that 







The reduction relies on two other functions: 
\begin{itemize}
\item
The $\counterred{\bound}$ reduction is a generalization of 
The goal of \theeplayer is to keep these counters below $\bound$.

\rfm{Moved here}


Here, $\bound$ is a parameter of the reduction, and for completeness we will need it to be $n$-fold exponential in the size of the given game $\game$. 
Let $\ap{\polyred{}}{\game}$ genote the safety game obtained for this bound.


%in the sense that a winning strategy in one implies a winning strategy in the other for \theeplayer.
In particular, we need the following lemma.


% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
This allows us to argue that \theeplayer wins the parity $\game$ iff they win the safety game $\gamec$.
}

==> polynomial_unused.tex <==
In this case, $\encodingalphabet{\rank}$ are the characters needed to index the encoding.

%where the top of the stack is on the left. 
%Note that $\indexalphabet^\ast$ is a very specific sequence of characters.
%In particular,

%Initially, we require \theaplayer to build the correct stack, which contains only the character
%$\tup{\chainit, 0, \ldots, 0}$.
%This is enforced by an initial control state.
%After the correct initial configuration has been built, the simulation is .


The state $\controlinit'$ is the initial control state and indicates that \theaplayer must build the correct initial stack.
The owner of the control state does not matter.
We give it to \theaplayer.

The state $\eover$ indicates a loss for \theeplayer.
The owners of the control state does not matter.
We give it to \theaplayer.

Finally, $\controlscw$ are the control states needed by Cachat and Walukiewicz to implement $\countercheck{\rank}$ and $\equalscheck{\rank}$.
Their owners are given by Cachat and Walukiewicz (or more precisely, their dual).


 as well as a new initial character.

 \set{\chainit'} \cup
    Moreover, there i s
    If $\genop=\pop{1}$, the following rule exists for all $\linkchar{\opord}\in \linkalphabet$. 
    If $\genop=\collapse{\opord}$, we only have it for $\linkchar{\opord}$ with $\opord$ as required by the collapse:
    \[
        \tup{\tup{\genop, \rank, \control'},
             \linkchar{\opord},
             \genop,
             \controlincnoa{\rank}{\control'}}\ .
    \]


 

==> preliminaries_unused.tex <==
Afterwards we 
The stack operations defined below, create copies of sub-stacks.
 formally after the definition of stacks.


is that It may be helpful to think about a collTo give an intut 
This will be captured by exec
 These operations 
Besides the pop operations, which areAdditionally, coll and of order $\opord>1$ of any order of arbitrary order on a higher-order st
The following operations may be performed on an order-$\cpdsord$ collapsible stack.

 where the links are given as superscripts:

 Collapse links are created by the
$\cpush{\cha}{\opord}$
operations, which add a character to the top of a given stack $\stackw$ with a link pointing to
$\ap{\pop{\opord}}{\stackw}$.
We set


%For full introduction, we refer the reader to Hague\etal~\cite{HMOS08}.


%Intuitively, this is the context (of the corresponding order) in which the character is created.
%To be more precise, the link is to the order-$\opord$ stack that is the result of performing a $\pop{k}$ on the current $(\opord+1)$-stack.
%We discuss the semantics in detail in a moment
%The semantics is made precise below.

%This means the collapse operation restores the context (of the corresponding order) in which the character was created.

        %\sbrac{\sbrac{\annot{\chd}{\tup{1,1}} \annot{\che}{\tup{1,1}}}{1}}{2}
        %\sbrac{\sbrac{\annot{\chd}{\tup{1,1}} \annot{\che}{\tup{1,1}}}{1}}{2}
}

\mh{TODO: add initial configuration}


 a rule.  %If $\ap{\owner}{\control} = \eplayer$, 
%then \theeplayer chooses, otherwise \theaplayer chooses a rule.
This rule is applied, giving a transition to the next configuration
$\config{\control'}{\stackw'}$. 
This leads to an infinite play, a sequence

%where $\cpdstran$ is the transition relation from above. 
 % formed where, for all $\idxi$,
%$\config{\control_\idxi}{\stackw_\idxi}
% \cpdstran
% \config{\control_{\idxi+1}}{\stackw_{\idxi+1}}$.
}



% to reflect the information tracked by the construction used in the proofs.
%Note also that Hague\etal 
%Hague\etal only provide a function $\ranks$ for order-$2$ and above.
%It is trivial to extend it to include order-$1$ and links.



% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------
% -------------------------------------------------------------------------------

\begin{remark}
\end{remark}


==> stuff.tex <==
%
% Stuff
%

\let\leq\leqslant
\let\geq\geqslant
\let\nleq\leqslant
\let\ngeq\ngeqslant

% separation rules
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

\theoremstyle{plain}
\newtheorem{proposition}[theorem]{Proposition}

